Safety-aware time-optimal motion planning with uncertain human state estimation

Human awareness in robot motion planning is crucial for seamless interaction with humans. Many existing techniques slow down, stop, or change the robot's trajectory locally to avoid collisions with humans. Although using the information on the human's state in the path planning phase could reduce future interference with the human's movements and make safety stops less frequent, such an approach is less widespread. This paper proposes a novel approach to embedding a human model in the robot's path planner. The method explicitly addresses the problem of minimizing the path execution time, including slowdowns and stops owed to the proximity of humans. For this purpose, it converts safety speed limits into configuration-space cost functions that drive the path's optimization. The costmap can be updated based on the observed or predicted state of the human. The method can handle deterministic and probabilistic representations of the human state and is independent of the prediction algorithm. Numerical and experimental results on an industrial collaborative cell demonstrate that the proposed approach consistently reduces the robot's execution time and avoids unnecessary safety speed reductions.

==> lambda_map.tex <==
\begin{tcbraster}[raster columns=3, raster equal height, raster column skip=0mm, raster row skip=0mm,
]
\begin{tcolorbox}[mybox={S}{helpful!50!internal}]
\begin{myitemize}
\item A
\item B
\item C
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={S}{helpful!50!internal}]
\begin{myitemize}
\item A
\item B
\item C
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={W}{harmful!50!internal}]
\begin{myitemize}
\item A
\item B
\item C
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={O}{helpful!50!external}]
\begin{myitemize}
\item A
\item B
\item C
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={}{SO}]
\begin{myitemize}
\item A
\item B
\item C
\item D
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={}{WO}]
\begin{myitemize}
\item A
\item B
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={T}{harmful!50!external}]
\begin{myitemize}
\item A
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={}{ST}]
\begin{myitemize}
\item A
\item B
\end{myitemize}
\end{tcolorbox}
\begin{tcolorbox}[mybox={}{WT}]
\begin{myitemize}
\item A
\item B
\item CCCCCCCCCC
\end{myitemize}
\end{tcolorbox}
\end{tcbraster}
